Plant Taxonomy Meets Plant Counting: A Fine-Grained, Taxonomic Dataset for Counting Hundreds of Plant Species

Visually cataloging and quantifying the natural world requires pushing the boundaries of both detailed visual classification and counting at scale. Despite significant progress, particularly in crowd and traffic analysis, the fine-grained, taxonomy-aware plant counting remains underexplored in vision. In contrast to crowds, plants exhibit nonrigid morphologies and physical appearance variations across growth stages and environments. To fill this gap, we present TPC-268, the first plant counting benchmark incorporating plant taxonomy. Our dataset couples instance-level point annotations with Linnaean labels (kingdom -> species) and organ categories, enabling hierarchical reasoning and species-aware evaluation. The dataset features 10,000 images with 678,050 point annotations, includes 268 countable plant categories over 242 plant species in Plantae and Fungi, and spans observation scales from canopy-level remote sensing imagery to tissue-level microscopy. We follow the problem setting of class-agnostic counting (CAC), provide taxonomy-consistent, scale-aware data splits, and benchmark state-of-the-art regression- and detection-based CAC approaches. By capturing the biodiversity, hierarchical structure, and multi-scale nature of botanical and mycological taxa, TPC-268 provides a biologically grounded testbed to advance fine-grained class-agnostic counting. Dataset and code are available at https://github.com/tiny-smart/TPC-268.

==> sec/acknowledgement.tex <==
% \section*{Acknowledgement}
% \noindent\textbf{Acknowledgement.} This work is supported in part by the National Natural Science Foundation of China under Grant No.~62576146 and in part by the HUST Undergraduate Natural Science Foundation under Grant No.~62500034.

==> sec/sup_mapping_table.tex <==
\tablecaption{Mapping table}\label{tab:mytable}

\begin{center}
\footnotesize
\tablehead{\toprule \textbf{Category} & \textbf{ID} \\ \midrule}
\tabletail{
% \midrule
\multicolumn{2}{r}{{...}} \\
\bottomrule
}
\tablelasttail{
\bottomrule
}
\begin{supertabular}{p{0.9\linewidth}c}
\textit{Kingdom} &  \\ \midrule
Plantae & 1 \\ 
Fungi & 2 \\ 
\midrule \textit{Phylum} &  \\ \midrule
Tracheophyta & 1 \\ 
Basidiomycota & 2 \\ 
\midrule \textit{Class} &  \\ \midrule
Magnoliopsida & 1 \\ 
Agaricomycetes & 2 \\ 
Liliopsida & 3 \\ 
Polypodiopsida & 4 \\ 
\midrule \textit{Order} &  \\ \midrule
Malvales & 1 \\ 
Fabales & 2 \\ 
Sapindales & 3 \\ 
Caryophyllales & 4 \\ 
Ericales & 5 \\ 
Boraginales & 6 \\ 
Agaricales & 7 \\ 
Asparagales & 8 \\ 
Poales & 9 \\ 
Myrtales & 10 \\ 
Ranunculales & 11 \\ 
Magnoliales & 12 \\ 
Asterales & 13 \\ 
Rosales & 14 \\ 
Oxalidales & 15 \\ 
Proteales & 16 \\ 
Cucurbitales & 17 \\ 
Brassicales & 18 \\ 
Apiales & 19 \\ 
Solanales & 20 \\ 
Fagales & 21 \\ 
Malpighiales & 22 \\ 
Arecales & 23 \\ 
Gentianales & 24 \\ 
Cornales & 25 \\ 
Polypodiales & 26 \\ 
Lamiales & 27 \\ 
Aquifoliales & 28 \\ 
Saxifragales & 29 \\ 
Zingiberales & 30 \\ 
Laurales & 31 \\ 
Zygophyllales & 32 \\ 
Liliales & 33 \\ 
Vitales & 34 \\ 
Santalales & 35 \\ 
\midrule \textit{Family} &  \\ \midrule
Malvaceae & 1 \\ 
Fabaceae & 2 \\ 
Sapindaceae & 3 \\ 
Amaranthaceae & 4 \\ 
Actinidiaceae & 5 \\ 
Boraginaceae & 6 \\ 
Agaricaceae & 7 \\ 
Bolbitiaceae & 8 \\ 
Amaryllidaceae & 9 \\ 
Anacardiaceae & 10 \\ 
Bromeliaceae & 11 \\ 
Melastomataceae & 12 \\ 
Ranunculaceae & 13 \\ 
Annonaceae & 14 \\ 
Caryophyllaceae & 15 \\ 
Asteraceae & 16 \\ 
Moraceae & 17 \\ 
Asparagaceae & 18 \\ 
Oxalidaceae & 19 \\ 
Cactaceae & 20 \\ 
Meliaceae & 21 \\ 
Proteaceae & 22 \\ 
Cucurbitaceae & 23 \\ 
Burseraceae & 24 \\ 
Brassicaceae & 25 \\ 
Simaroubaceae & 26 \\ 
Apiaceae & 27 \\ 
Cannabaceae & 28 \\ 
Solanaceae & 29 \\ 
Caricaceae & 30 \\ 
Juglandaceae & 31 \\ 
Salicaceae & 32 \\ 
Fagaceae & 33 \\ 
Rutaceae & 34 \\ 
Arecaceae & 35 \\ 
Rubiaceae & 36 \\ 
Cordiaceae & 37 \\ 
Betulaceae & 38 \\ 
Rosaceae & 39 \\ 
Primulaceae & 40 \\ 
Hydrangeaceae & 41 \\ 
Ebenaceae & 42 \\ 
Thymelaeaceae & 43 \\ 
Aizoaceae & 44 \\ 
Polypodiaceae & 45 \\ 
Cyperaceae & 46 \\ 
Heliotropiaceae & 47 \\ 
Frankeniaceae & 48 \\ 
Oleaceae & 49 \\ 
Clusiaceae & 50 \\ 
Polemoniaceae & 51 \\ 
Lardizabalaceae & 52 \\ 
Aquifoliaceae & 53 \\ 
Convolvulaceae & 54 \\ 
Magnoliaceae & 55 \\ 
Euphorbiaceae & 56 \\ 
Sapotaceae & 57 \\ 
Plantaginaceae & 58 \\ 
Lamiaceae & 59 \\ 
Saxifragaceae & 60 \\ 
Moringaceae & 61 \\ 
Musaceae & 62 \\ 
Myricaceae & 63 \\ 
Nelumbonaceae & 64 \\ 
Nepenthaceae & 65 \\ 
Ericaceae & 66 \\ 
Nyssaceae & 67 \\ 
Poaceae & 68 \\ 
Passifloraceae & 69 \\ 
Lauraceae & 70 \\ 
Pleurotaceae & 71 \\ 
Lythraceae & 72 \\ 
Salvadoraceae & 73 \\ 
Myrtaceae & 74 \\ 
Bignoniaceae & 75 \\ 
Zygophyllaceae & 76 \\ 
Liliaceae & 77 \\ 
Ulmaceae & 78 \\ 
Dipterocarpaceae & 79 \\ 
Apocynaceae & 80 \\ 
Vitaceae & 81 \\ 
Olacaceae & 82 \\ 
Rhamnaceae & 83 \\ 
\midrule \textit{Genus} &  \\ \midrule
Abelmoschus & 1 \\ 
Abutilon & 2 \\ 
Acacia & 3 \\ 
Vachellia & 4 \\ 
Acer & 5 \\ 
Achyranthes & 6 \\ 
Psilotrichum & 7 \\ 
Cyathula & 8 \\ 
Centrostachys & 9 \\ 
Acmispon & 10 \\ 
Actinidia & 11 \\ 
Adelinia & 12 \\ 
Adenanthera & 13 \\ 
Agaricus & 14 \\ 
Cyclocybe & 15 \\ 
Allium & 16 \\ 
Amphicarpaea & 17 \\ 
Anacardium & 18 \\ 
Ananas & 19 \\ 
Anarthrophyllum & 20 \\ 
Andesanthus & 21 \\ 
Anemonastrum & 22 \\ 
Annona & 23 \\ 
Arachis & 24 \\ 
Minuartia & 25 \\ 
Arrowsmithia & 26 \\ 
Artocarpus & 27 \\ 
Asparagus & 28 \\ 
Averrhoa & 29 \\ 
Aylostera & 30 \\ 
Azadirachta & 31 \\ 
Banksia & 32 \\ 
Benincasa & 33 \\ 
Beta & 34 \\ 
Boswellia & 35 \\ 
Brassica & 36 \\ 
Brucea & 37 \\ 
Bupleurum & 38 \\ 
Canarium & 39 \\ 
Cannabis & 40 \\ 
Capsicum & 41 \\ 
Carica & 42 \\ 
Carya & 43 \\ 
Casearia & 44 \\ 
Castanea & 45 \\ 
Ceratonia & 46 \\ 
Chaetogastra & 47 \\ 
Cheniella & 48 \\ 
Chrysanthemum & 49 \\ 
Cicer & 50 \\ 
Citrullus & 51 \\ 
Citrus & 52 \\ 
Clausena & 53 \\ 
Cocos & 54 \\ 
Coffea & 55 \\ 
Conopodium & 56 \\ 
Coprinus & 57 \\ 
Cordeauxia & 58 \\ 
Cordia & 59 \\ 
Corylus & 60 \\ 
Crataegus & 61 \\ 
Crotalaria & 62 \\ 
Cucumis & 63 \\ 
Cucurbita & 64 \\ 
Cyanothamnus & 65 \\ 
Cyclamen & 66 \\ 
Dalbergia & 67 \\ 
Daucus & 68 \\ 
Deutzia & 69 \\ 
Dianthus & 70 \\ 
Didymanthus & 71 \\ 
Diospyros & 72 \\ 
Dirca & 73 \\ 
Eucephalus & 74 \\ 
Donnellsmithia & 75 \\ 
Drosanthemum & 76 \\ 
Aglaomorpha & 77 \\ 
Durio & 78 \\ 
Eleocharis & 79 \\ 
Epiphyllum & 80 \\ 
Eriolarynx & 81 \\ 
Eryngium & 82 \\ 
Euploca & 83 \\ 
Fenestraria & 84 \\ 
Ficus & 85 \\ 
Fragaria & 86 \\ 
Frankenia & 87 \\ 
Fraxinus & 88 \\ 
Garcinia & 89 \\ 
Gelasia & 90 \\ 
Scorzonera & 91 \\ 
Giliastrum & 92 \\ 
Glycine & 93 \\ 
Helianthus & 94 \\ 
Holboellia & 95 \\ 
Hypochaeris & 96 \\ 
Ilex & 97 \\ 
Ipomoea & 98 \\ 
Jacobaea & 99 \\ 
Jaumea & 100 \\ 
Juglans & 101 \\ 
Lablab & 102 \\ 
Lactuca & 103 \\ 
Lagenaria & 104 \\ 
Aglaia & 105 \\ 
Laserpitium & 106 \\ 
Leptosiphon & 107 \\ 
Litchi & 108 \\ 
Lordhowea & 109 \\ 
Luffa & 110 \\ 
Lycium & 111 \\ 
Magnolia & 112 \\ 
Malus & 113 \\ 
Mangifera & 114 \\ 
Manihot & 115 \\ 
Manilkara & 116 \\ 
Matourea & 117 \\ 
Mentha & 118 \\ 
Asimitellaria & 119 \\ 
Momordica & 120 \\ 
Mononeuria & 121 \\ 
Moringa & 122 \\ 
Morus & 123 \\ 
Musa & 124 \\ 
Morella & 125 \\ 
Narcissus & 126 \\ 
Nelumbo & 127 \\ 
Nepenthes & 128 \\ 
Nephelium & 129 \\ 
Nicotiana & 130 \\ 
Vaccinium & 131 \\ 
Nyssa & 132 \\ 
Opuntia & 133 \\ 
Ormosia & 134 \\ 
Oryza & 135 \\ 
Passiflora & 136 \\ 
Peniocereus & 137 \\ 
Pentanema & 138 \\ 
Persea & 139 \\ 
Phaseolus & 140 \\ 
Phoenix & 141 \\ 
Pilosocereus & 142 \\ 
Pisum & 143 \\ 
Pleurotus & 144 \\ 
Populus & 145 \\ 
Potentilla & 146 \\ 
Prunus & 147 \\ 
Pseudopodospermum & 148 \\ 
Punica & 149 \\ 
Pyrus & 150 \\ 
Quercus & 151 \\ 
Rabelera & 152 \\ 
Raphanus & 153 \\ 
Ricinus & 154 \\ 
Rosa & 155 \\ 
Rubus & 156 \\ 
Salix & 157 \\ 
Salvadora & 158 \\ 
Sandoricum & 159 \\ 
Sapindus & 160 \\ 
Schinus & 161 \\ 
Selenicereus & 162 \\ 
Senegalia & 163 \\ 
Silene & 164 \\ 
Siraitia & 165 \\ 
Sohmaea & 166 \\ 
Solanum & 167 \\ 
Sorghum & 168 \\ 
Spondias & 169 \\ 
Stauntonia & 170 \\ 
Syzygium & 171 \\ 
Tamarindus & 172 \\ 
Tanaecium & 173 \\ 
Theobroma & 174 \\ 
Tibetiodes & 175 \\ 
Aster & 176 \\ 
Toiyabea & 177 \\ 
Tribulus & 178 \\ 
Trichosanthes & 179 \\ 
Triticum & 180 \\ 
Tulipa & 181 \\ 
Ulmus & 182 \\ 
Vatica & 183 \\ 
Vernicia & 184 \\ 
Vincetoxicum & 185 \\ 
Vitis & 186 \\ 
Walsholaria & 187 \\ 
Pascalia & 188 \\ 
Wissadula & 189 \\ 
Ximenia & 190 \\ 
Zea & 191 \\ 
Ziziphus & 192 \\ 
\midrule \textit{Species} &  \\ \midrule
Abelmoschus esculentus & 1 \\ 
Abutilon indicum & 2 \\ 
Acacia aspera & 3 \\ 
Vachellia tortilis & 4 \\ 
Acer rubrum & 5 \\ 
Achyranthes aspera & 6 \\ 
Psilotrichum argenteum & 7 \\ 
Cyathula mucronata & 8 \\ 
Psilotrichum recurvatum & 9 \\ 
Centrostachys stricta & 10 \\ 
Acmispon decumbens & 11 \\ 
Acmispon neomexicanus & 12 \\ 
Acmispon tomentosus & 13 \\ 
Actinidia deliciosa & 14 \\ 
Adelinia grandis & 15 \\ 
Adenanthera pavonina & 16 \\ 
Agaricus bisporus & 17 \\ 
Agaricus blazei & 18 \\ 
Cyclocybe aegerita & 19 \\ 
Allium cepa & 20 \\ 
Allium sativum & 21 \\ 
Amphicarpaea elliptica & 22 \\ 
Anacardium occidentale & 23 \\ 
Ananas comosus & 24 \\ 
Anarthrophyllum desideratum & 25 \\ 
Andesanthus lepidotus & 26 \\ 
Anemonastrum deltoideum & 27 \\ 
Annona reticulata & 28 \\ 
Annona squamosa & 29 \\ 
Arachis hypogaea & 30 \\ 
Minuartia paludicola & 31 \\ 
Arrowsmithia tenuifolia & 32 \\ 
Artocarpus heterophyllus & 33 \\ 
Asparagus officinalis & 34 \\ 
Averrhoa carambola & 35 \\ 
Aylostera pygmaea & 36 \\ 
Azadirachta indica & 37 \\ 
Banksia ashbyi & 38 \\ 
Benincasa hispida & 39 \\ 
Beta vulgaris & 40 \\ 
Boswellia sacra & 41 \\ 
Brassica napus & 42 \\ 
Brucea javanica & 43 \\ 
Bupleurum ranunculoides & 44 \\ 
Canarium album & 45 \\ 
Cannabis sativa & 46 \\ 
Capsicum annuum & 47 \\ 
Carica papaya & 48 \\ 
Carya cathayensis & 49 \\ 
Carya illinoinensis & 50 \\ 
Carya ovata & 51 \\ 
Casearia yucatanensis & 52 \\ 
Castanea mollissima & 53 \\ 
Ceratonia siliqua & 54 \\ 
Chaetogastra herbacea & 55 \\ 
Chaetogastra paratropica & 56 \\ 
Cheniella corymbosa & 57 \\ 
Cheniella glauca & 58 \\ 
Chrysanthemum × morifolium & 59 \\ 
Cicer arietinum & 60 \\ 
Citrullus lanatus & 61 \\ 
Citrus × limon & 62 \\ 
Citrus sinensis & 63 \\ 
Citrus tangerina & 64 \\ 
Clausena lansium & 65 \\ 
Cocos nucifera & 66 \\ 
Coffea arabica & 67 \\ 
Conopodium majus & 68 \\ 
Coprinus comatus & 69 \\ 
Cordeauxia edulis & 70 \\ 
Cordia sinensis & 71 \\ 
Corylus heterophylla & 72 \\ 
Crataegus pinnatifida & 73 \\ 
Crotalaria magaliesbergensis & 74 \\ 
Cucumis anguria & 75 \\ 
Cucumis melo & 76 \\ 
Cucumis sativus & 77 \\ 
Cucurbita maxima & 78 \\ 
Cucurbita pepo & 79 \\ 
Cyanothamnus coerulescens & 80 \\ 
Cyanothamnus nanus & 81 \\ 
Cyanothamnus polygalifolius & 82 \\ 
Cyclamen creticum & 83 \\ 
Cyclamen hederifolium & 84 \\ 
Dalbergia brownei & 85 \\ 
Daucus carota & 86 \\ 
Deutzia rugulosa & 87 \\ 
Dianthus caryophyllus & 88 \\ 
Didymanthus littoreus & 89 \\ 
Didymanthus trilobus & 90 \\ 
Diospyros kaki & 91 \\ 
Dirca palustris & 92 \\ 
Eucephalus breweri & 93 \\ 
Eucephalus engelmannii & 94 \\ 
Eucephalus ledophyllus & 95 \\ 
Donnellsmithia juncea & 96 \\ 
Drosanthemum calcareum & 97 \\ 
Aglaomorpha fortunei & 98 \\ 
Durio zibethinus & 99 \\ 
Eleocharis dulcis & 100 \\ 
Epiphyllum oxypetalum & 101 \\ 
Eriolarynx australis & 102 \\ 
Eryngium carlinae & 103 \\ 
Euploca foliosissima & 104 \\ 
Fenestraria rhopalophylla & 105 \\ 
Ficus carica & 106 \\ 
Fragaria × ananassa & 107 \\ 
Frankenia salsoloides & 108 \\ 
Fraxinus excelsior & 109 \\ 
Garcinia mangostana & 110 \\ 
Gelasia cretica & 111 \\ 
Gelasia ensifolia & 112 \\ 
Scorzonera filifolia & 113 \\ 
Giliastrum rigidulum & 114 \\ 
Glycine max & 115 \\ 
Helianthus annuus & 116 \\ 
Holboellia latifolia & 117 \\ 
Hypochaeris valdesii & 118 \\ 
Ilex opaca & 119 \\ 
Ipomoea batatas & 120 \\ 
Jacobaea taitungensis & 121 \\ 
Jaumea ciliata & 122 \\ 
Juglans regia & 123 \\ 
Lablab purpureus & 124 \\ 
Lactuca sativa & 125 \\ 
Lagenaria siceraria & 126 \\ 
Aglaia parasitica & 127 \\ 
Laserpitium gallicum & 128 \\ 
Leptosiphon nuttallii & 129 \\ 
Litchi chinensis & 130 \\ 
Lordhowea amygdalifolia & 131 \\ 
Lordhowea velleioides & 132 \\ 
Luffa aegyptiaca & 133 \\ 
Lycium barbarum & 134 \\ 
Magnolia denudata & 135 \\ 
Malus domestica & 136 \\ 
Mangifera indica & 137 \\ 
Manihot esculenta & 138 \\ 
Manilkara zapota & 139 \\ 
Matourea azurea & 140 \\ 
Mentha canadensis & 141 \\ 
Asimitellaria formosana & 142 \\ 
Momordica charantia & 143 \\ 
Mononeuria caroliniana & 144 \\ 
Moringa oleifera & 145 \\ 
Morus alba & 146 \\ 
Musa × paradisiaca & 147 \\ 
Morella pensylvanica & 148 \\ 
Narcissus pseudonarcissus & 149 \\ 
Nelumbo nucifera & 150 \\ 
Nepenthes × ventrata & 151 \\ 
Nephelium lappaceum & 152 \\ 
Nicotiana tabacum & 153 \\ 
Vaccinium arisanense & 154 \\ 
Nyssa sylvatica & 155 \\ 
Opuntia ficus-indica & 156 \\ 
Ormosia ormondii & 157 \\ 
Oryza sativa & 158 \\ 
Passiflora edulis & 159 \\ 
Peniocereus viperinus & 160 \\ 
Pentanema britannica & 161 \\ 
Pentanema conyzae & 162 \\ 
Pentanema helenioides & 163 \\ 
Pentanema orientale & 164 \\ 
Pentanema spiraeifolium & 165 \\ 
Persea americana & 166 \\ 
Phaseolus vulgaris & 167 \\ 
Phoenix dactylifera & 168 \\ 
Pilosocereus curtisii & 169 \\ 
Pisum sativum & 170 \\ 
Pleurotus eryngii & 171 \\ 
Populus tomentosa & 172 \\ 
Potentilla indica & 173 \\ 
Prunus armeniaca & 174 \\ 
Prunus avium & 175 \\ 
Prunus davidiana & 176 \\ 
Prunus domestica & 177 \\ 
Prunus dulcis & 178 \\ 
Prunus persica & 179 \\ 
Pseudopodospermum hispanicum & 180 \\ 
Punica granatum & 181 \\ 
Pyrus communis & 182 \\ 
Quercus michauxii & 183 \\ 
Quercus nigra & 184 \\ 
Quercus pagoda & 185 \\ 
Quercus phellos & 186 \\ 
Quercus shumardii & 187 \\ 
Quercus stellata & 188 \\ 
Quercus texana & 189 \\ 
Rabelera holostea & 190 \\ 
Raphanus raphanistrum & 191 \\ 
Raphanus sativus & 192 \\ 
Ricinus communis & 193 \\ 
Rosa rugosa & 194 \\ 
Rubus idaeus & 195 \\ 
Salix babylonica & 196 \\ 
Salvadora persica & 197 \\ 
Sandoricum koetjape & 198 \\ 
Sapindus saponaria & 199 \\ 
Schinus molle & 200 \\ 
Selenicereus undatus & 201 \\ 
Senegalia senegal & 202 \\ 
Silene stellata & 203 \\ 
Siraitia grosvenorii & 204 \\ 
Sohmaea laxiflora & 205 \\ 
Solanum lycopersicum & 206 \\ 
Solanum melongena & 207 \\ 
Solanum torvum & 208 \\ 
Solanum tuberosum & 209 \\ 
Sorghum bicolor & 210 \\ 
Spondias dulcis & 211 \\ 
Stauntonia chinensis & 212 \\ 
Syzygium jambos & 213 \\ 
Syzygium samarangense & 214 \\ 
Tamarindus indica & 215 \\ 
Tanaecium dichotomum & 216 \\ 
Theobroma cacao & 217 \\ 
Tibetiodes asteroides & 218 \\ 
Aster flaccidus & 219 \\ 
Toiyabea peirsonii & 220 \\ 
Tribulus terrestris & 221 \\ 
Trichosanthes cucumerina & 222 \\ 
Triticum aestivum & 223 \\ 
Tulipa gesneriana & 224 \\ 
Ulmus alata & 225 \\ 
Ulmus americana & 226 \\ 
Vaccinium corymbosum & 227 \\ 
Vaccinium myrtillus & 228 \\ 
Vaccinium stamineum & 229 \\ 
Vaccinium vitis-idaea & 230 \\ 
Vatica mangachapoi & 231 \\ 
Vernicia fordii & 232 \\ 
Vincetoxicum koi & 233 \\ 
Vitis vinifera & 234 \\ 
Walsholaria magniflora & 235 \\ 
Walsholaria muelleri & 236 \\ 
Pascalia mexicana & 237 \\ 
Wissadula excelsior & 238 \\ 
Ximenia caffra & 239 \\ 
Zea mays & 240 \\ 
Ziziphus jujuba & 241 \\ 
Ziziphus mauritiana & 242 \\ 
\end{supertabular}
\end{center}
